Cyclic Nonassociative Bilinear Logic With Additive Constants as Extension of Full Nonassociative Lambek Calculus

Cyclic Linear Logic (CyMALL, CyBL) is a compromise between Commutative Linear Logic (MALL) and Noncommutative Linear Logic (Bilinear Logic, BL). We do not admit commutativity of the tensor, but we still admit only one De Morgan negation. MALL and its variants are natural extensions of Full Lambek Calculus (FL). Abrusci proved that CyBL is not a conservative extension of FL, if we admit additive constants in these logics. In this paper we show that Cyclic Nonassociative Bilinear Logic (CyNBL) with both additive constants is a strongly conservative extension of Full Nonassociative Lambek Calculus with only one additive constant - the upper bound - and that this holds even in the presence of an arbitrary set of nonlogical axioms.

==> eptcsdata.tex <==
\providecommand{\firstpage}{151}
\providecommand{\publicationstatus}{A. Indrzejczak, T. Jarmu\.zek, M. Klonowski, \& M. Zawidzki (Eds.):\\ Twelfth International Conference on\\ Non-Classical Logics. Theory and Applications (NCL'26)\\
EPTCS 455, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.455.12}{10.4204/EPTCS.455.12}}
\pdfoutput=1

